Decentralized Learning of Tree-Structured Gaussian Graphical Models from Noisy Data

This paper studies the decentralized learning of tree-structured Gaussian graphical models (GGMs) from noisy data. In decentralized learning, data set is distributed across different machines (sensors), and GGMs are widely used to model complex networks such as gene regulatory networks and social networks. The proposed decentralized learning uses the Chow-Liu algorithm for estimating the tree-structured GGM. In previous works, upper bounds on the probability of incorrect tree structure recovery were given mostly without any practical noise for simplification. While this paper investigates the effects of three common types of noisy channels: Gaussian, Erasure, and binary symmetric channel. For Gaussian channel case, to satisfy the failure probability upper bound $\delta > 0$ in recovering a $d$-node tree structure, our proposed theorem requires only $\mathcal{O}(\log(\frac{d}{\delta}))$ samples for the smallest sample size ($n$) comparing to the previous literature \cite{Nikolakakis} with $\mathcal{O}(\log^4(\frac{d}{\delta}))$ samples by using the positive correlation coefficient assumption that is used in some important works in the literature. Moreover, the approximately bounded Gaussian random variable assumption does not appear in \cite{Nikolakakis}. Given some knowledge about the tree structure, the proposed Algorithmic Bound will achieve obviously better performance with small sample size (e.g., $< 2000$) comparing with formulaic bounds. Finally, we validate our theoretical results by performing simulations on synthetic data sets.

==> Decentralized Tree Learning/extra.tex <==
\textbf{Description of Algorithmic Bound:} Algorithmic Bound is given in Algorithm \ref{algorithm2} and Algorithm \ref{algorithm3}. The main body of the program is from lines 1-4 in Algorithm \ref{algorithm2} where the empty arrays are defined and Break, Compute, and Bound functions are called to break the tree if it is large, compute the upper bounds on the subtrees and neighborhoods of an edge, and sum the upper bounds, respectively.

Lines 1-13 define Break function in Algorithm \ref{algorithm3} which breaks the tree if the number of nodes is greater than or equal to 10 (heuristic criterion), and put the subtrees and the neighborhoods of nodes (i.e., the nodes of the potential edge) into arrays $A_1$ and $A_2$, respectively. It calls FindEdge function (lines 32-37) to look for the potential edge such that the subtrees are almost half. The stopping criterion (line 4) is based on the prefactor $d^3$. For $d\geq10$, Theorem \ref{theorem2} performance becomes loose for small size data set, therefore, it is needed to break the tree into subtrees. Hence, it is reasonable to have this criterion. In addition, this criterion does not enhance the time complexity of Algorithmic Bound.

Compute function is defined in lines 14-24 which computes the upper bounds on subtrees and neighborhoods based on Theorem \ref{theorem2} and the results are stored in arrays $U_1$ and $U_2$.

The bound function is given in lines 25-31 which sums the upper bounds on the subtrees and neighborhoods and returns the final bound on the probability of incorrect recovery of tree structure.


\begin{algorithm}[hbt]
\LinesNumbered
\SetAlgoLined
%\DontPrintSemicolon
\KwIn{$T_p(V, E)$ (tree-structured graph), $\beta = \rho_e - \rho_{e'}$ (difference of the correlation coefficients), $a_M, b_M$ (lower and upper bounds respectively on the random variables in Theorem \ref{theorem2}), and a number of samples $n$}
\KwOut{Upper bound on incorrect tree recovery probability $Pr(\hat{T}_p \neq T_p)$}
%\NoNumber{A}
{
Initialization: $A_1$, $A_2$, $U_1$, $U_2$ one dimensional arrays\;
Call Break($T_p$) \tcp*[r]{Calling Break function for tree graph}
Call Compute($A_1$, $A_2$, $\beta$, $a_M$, $b_M$, $n$) \tcp*[r]{compute the bound for each subtree and potential edges}
$Upperbound$ = Bound($U_1$, $U_2$) \tcp*[r]{sum all the bounds}
}
\caption{Algorithmic Bound based on Algorithm 3}
\label{algorithm2}
\end{algorithm}

\begin{algorithm}
\LinesNumbered
%\setcounter{AlgoLine}{4}
\SetAlgoLined
%\textbf{Functions:}

\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{FB}{Break}
 \Fn{\FB{$T_p$}}{
 \KwIn{Tree $T_p$}
 \KwOut{Save the outputs in arrays $A_1$ and $A_2$}
 \tcp*[r]{this function breaks the complete tree into subtrees}
    $d = |V|$ (number of nodes)   \tcp*[r]{$T_p(V, E)$}
    \If{$d \geq 10$}{
    [$g_{ij}$, $N(i)$, $N(j)$] = Call FindEdge($T_p$) \tcp*[r]{Finding an edge $g_{ij}$ and set of neighbors of node i (e.g., $N(i)$) and node j}
    Remove $g_{ij}$\;
    Put subtrees $T_1$ and $T_2$ in array $A_1$\;
    Put sets of neighbors of node $i$ $N(i)$ and node $j $ $N(j)$ in array $A_2$\;
    }
    \ForEach{$T_l \in A_1 $}{
    Call Break($T_l$)\tcp*[r]{recursively break the subtrees $T_l$ in array $A_1$}
    }
}
\textbf{End} Break

\SetKwFunction{FC}{Compute}
\Fn{\FC{$A_1$, $A_2$, $\beta$, $a_M$, $b_M$, $n$}}{
\KwIn{Arrays $A_1$ and $A_2$, $\beta$ (difference of the correlation coefficients), $a_M, b_M$ (lower and upper bounds respectively on the random variables in Theorem \ref{theorem2}), a number of samples $n$}
\KwOut{Save the upper bounds in array $U_1$ and $U_2$}
\ForEach{$T_l \in A_1 $}{
    $T_l$  \tcp*[r]{subtrees $T_l(V_l, E_l)$}
    $u = d_l^3 e^{-\frac{2n\beta^2}{(b_M - a_M)^2}}$ \tcp*[r]{computing upper bounds for each subtree using Theorem \ref{theorem2} and $d_l = |V_l|$}
    Put the upper bound $u$ in array $U_1$\;
    }
\ForEach{$ N(q) \in A_2 $}{
    $v = N(q) e^{-\frac{2n\beta^2}{(b_M - a_M)^2}}$ \tcp*[r]{computing upper bound for a set of neighbors of node $q$ in array $A_2$}
    Put the upper bound $v$ in array $U_2$\;
    }
}
\textbf{End} Compute

\SetKwFunction{FJ}{Bound}
\Fn{\FJ{$U_1$, $U_2$}}{
\KwIn{Arrays of upper bounds $U_1$ and $U_2$}
\KwOut{Sum of upper bounds in array $U_1$ and $U_2$}
Find the size of array $U_1$ \tcp*[r]{since $size(U_1) = size(U_2)$}

\For{$c = 1$ to $size(U_1)$}{
sum $\leftarrow$ sum + $U_1[c] + U_2[c]$ \tcp*[r]{sum of upper bounds}
}
\Return sum
}
\textbf{End} Bound

\caption{Functions for Algorithm 2}
\label{algorithm3}
\end{algorithm}

\begin{algorithm}%[H]
\LinesNumbered
\setcounter{AlgoLine}{31}
\SetAlgoLined
%\textbf{Functions:}

\SetKwProg{Fn}{Function}{:}{}

\SetKwFunction{FF}{FindEdge}
\Fn{\FF{$T_p(V, E)$}}{
\KwIn{Tree $T_p$}
\KwOut{An edge $e_{ij}$ and sets of neighbors of node $i$ and node $j$ (e.g., $N(i)$ and $N(j)$)}
$d = |V|$ (number of nodes) \tcp*[r]{This function finds an edge and neighborhoods}
search an edge $e_{ij} \in E$ such that removal of $e_{ij}$ creates two subtrees $T_1$ and $T_2$ of $T$ with almost $\frac{1}{2}d$ nodes each\;
find $N(i)$ and $N(j)$\;
\Return [$e_{ij}$, $N(i)$, $N(j)$]
}
\textbf{End} FindEdge
\end{algorithm}

Following definitions are required to prove that Algorithmic Bound is correct.
\begin{definition}[Correlation decay property] \label{def2}
The Correlation Decay Property (CDP) states that the absolute value of the correlation coefficient between any two nodes decreases as the distance (the number of edges along the path between two nodes) between them increases \cite{F.Tan}.
\end{definition}
The dominant crossover event in tree-structured GGMs is defined in \cite{F.Tan}, \cite{Tavass}. The effect of this crossover event is as follows.
\begin{definition}[Impact of dominant errors]\label{def3}
An edge $e_{ij}$ is replaced with one of the candidate false edges: node $i$ is connected to one of the neighbors of node $j$ or vice versa.
\end{definition}

\subsubsection{Analysis of Algorithmic Bound}
First the time complexity of Algorithmic Bound (Algorithm \ref{algorithm2} and Algorithm \ref{algorithm3}) is discussed, and then proof of Algorithmic Bound correctness is provided by showing the validity of upper bound which is tighter than Theorem \ref{theorem2}.

\noindent \textbf{Time Complexity:} The overall time complexity of Algorithmic Bound (Algorithm 2 and Algorithm 3) is $\mathcal{O}(d)$ where $d$ is the number of nodes in a tree, which is dominated by the Break Function.

\noindent Time Complexity of Function Break: This function recursively breaks the tree with $d$ nodes in lines 10-11 of Algorithm \ref{algorithm3} where at each iteration the tree becomes almost half, hence, it takes $\mathcal{O}(\log d)$ time. While line 5 of Algorithm \ref{algorithm3} takes $\mathcal{O}(d)$ time due to FindEdge function. It has $\mathcal{O}(d)$ time complexity overall.

\begin{thm}[Algorithmic Bound on incorrect recovery probability] \label{theorem3}
Algorithmic Bound (Algorithm \ref{algorithm2}  and Algorithm \ref{algorithm3}) gives the valid upper bound on the incorrect tree structure recovery probability $Pr(\hat{T}_p \neq T_p)$, and it has $\mathcal{O}(d)$ time complexity where $d$ is the number of nodes in a tree graph.
\end{thm}
\begin{proof}
  Please see Appendix \ref{append5} for the proof of this theorem.
\end{proof}

==> extra.tex <==
\textbf{Description of Algorithmic Bound:} Algorithmic Bound is given in Algorithm \ref{algorithm2} and Algorithm \ref{algorithm3}. The main body of the program is from lines 1-4 in Algorithm \ref{algorithm2} where the empty arrays are defined and Break, Compute, and Bound functions are called to break the tree if it is large, compute the upper bounds on the subtrees and neighborhoods of an edge, and sum the upper bounds, respectively.

Lines 1-13 define Break function in Algorithm \ref{algorithm3} which breaks the tree if the number of nodes is greater than or equal to 10 (heuristic criterion), and put the subtrees and the neighborhoods of nodes (i.e., the nodes of the potential edge) into arrays $A_1$ and $A_2$, respectively. It calls FindEdge function (lines 32-37) to look for the potential edge such that the subtrees are almost half. The stopping criterion (line 4) is based on the prefactor $d^3$. For $d\geq10$, Theorem \ref{theorem2} performance becomes loose for small size data set, therefore, it is needed to break the tree into subtrees. Hence, it is reasonable to have this criterion. In addition, this criterion does not enhance the time complexity of Algorithmic Bound.

Compute function is defined in lines 14-24 which computes the upper bounds on subtrees and neighborhoods based on Theorem \ref{theorem2} and the results are stored in arrays $U_1$ and $U_2$.

The bound function is given in lines 25-31 which sums the upper bounds on the subtrees and neighborhoods and returns the final bound on the probability of incorrect recovery of tree structure.


\begin{algorithm}[hbt]
\LinesNumbered
\SetAlgoLined
%\DontPrintSemicolon
\KwIn{$T_p(V, E)$ (tree-structured graph), $\beta = \rho_e - \rho_{e'}$ (difference of the correlation coefficients), $a_M, b_M$ (lower and upper bounds respectively on the random variables in Theorem \ref{theorem2}), and a number of samples $n$}
\KwOut{Upper bound on incorrect tree recovery probability $Pr(\hat{T}_p \neq T_p)$}
%\NoNumber{A}
{
Initialization: $A_1$, $A_2$, $U_1$, $U_2$ one dimensional arrays\;
Call Break($T_p$) \tcp*[r]{Calling Break function for tree graph}
Call Compute($A_1$, $A_2$, $\beta$, $a_M$, $b_M$, $n$) \tcp*[r]{compute the bound for each subtree and potential edges}
$Upperbound$ = Bound($U_1$, $U_2$) \tcp*[r]{sum all the bounds}
}
\caption{Algorithmic Bound based on Algorithm 3}
\label{algorithm2}
\end{algorithm}

\begin{algorithm}
\LinesNumbered
%\setcounter{AlgoLine}{4}
\SetAlgoLined
%\textbf{Functions:}

\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{FB}{Break}
 \Fn{\FB{$T_p$}}{
 \KwIn{Tree $T_p$}
 \KwOut{Save the outputs in arrays $A_1$ and $A_2$}
 \tcp*[r]{this function breaks the complete tree into subtrees}
    $d = |V|$ (number of nodes)   \tcp*[r]{$T_p(V, E)$}
    \If{$d \geq 10$}{
    [$g_{ij}$, $N(i)$, $N(j)$] = Call FindEdge($T_p$) \tcp*[r]{Finding an edge $g_{ij}$ and set of neighbors of node i (e.g., $N(i)$) and node j}
    Remove $g_{ij}$\;
    Put subtrees $T_1$ and $T_2$ in array $A_1$\;
    Put sets of neighbors of node $i$ $N(i)$ and node $j $ $N(j)$ in array $A_2$\;
    }
    \ForEach{$T_l \in A_1 $}{
    Call Break($T_l$)\tcp*[r]{recursively break the subtrees $T_l$ in array $A_1$}
    }
}
\textbf{End} Break

\SetKwFunction{FC}{Compute}
\Fn{\FC{$A_1$, $A_2$, $\beta$, $a_M$, $b_M$, $n$}}{
\KwIn{Arrays $A_1$ and $A_2$, $\beta$ (difference of the correlation coefficients), $a_M, b_M$ (lower and upper bounds respectively on the random variables in Theorem \ref{theorem2}), a number of samples $n$}
\KwOut{Save the upper bounds in array $U_1$ and $U_2$}
\ForEach{$T_l \in A_1 $}{
    $T_l$  \tcp*[r]{subtrees $T_l(V_l, E_l)$}
    $u = d_l^3 e^{-\frac{2n\beta^2}{(b_M - a_M)^2}}$ \tcp*[r]{computing upper bounds for each subtree using Theorem \ref{theorem2} and $d_l = |V_l|$}
    Put the upper bound $u$ in array $U_1$\;
    }
\ForEach{$ N(q) \in A_2 $}{
    $v = N(q) e^{-\frac{2n\beta^2}{(b_M - a_M)^2}}$ \tcp*[r]{computing upper bound for a set of neighbors of node $q$ in array $A_2$}
    Put the upper bound $v$ in array $U_2$\;
    }
}
\textbf{End} Compute

\SetKwFunction{FJ}{Bound}
\Fn{\FJ{$U_1$, $U_2$}}{
\KwIn{Arrays of upper bounds $U_1$ and $U_2$}
\KwOut{Sum of upper bounds in array $U_1$ and $U_2$}
Find the size of array $U_1$ \tcp*[r]{since $size(U_1) = size(U_2)$}

\For{$c = 1$ to $size(U_1)$}{
sum $\leftarrow$ sum + $U_1[c] + U_2[c]$ \tcp*[r]{sum of upper bounds}
}
\Return sum
}
\textbf{End} Bound

\caption{Functions for Algorithm 2}
\label{algorithm3}
\end{algorithm}

\begin{algorithm}%[H]
\LinesNumbered
\setcounter{AlgoLine}{31}
\SetAlgoLined
%\textbf{Functions:}

\SetKwProg{Fn}{Function}{:}{}

\SetKwFunction{FF}{FindEdge}
\Fn{\FF{$T_p(V, E)$}}{
\KwIn{Tree $T_p$}
\KwOut{An edge $e_{ij}$ and sets of neighbors of node $i$ and node $j$ (e.g., $N(i)$ and $N(j)$)}
$d = |V|$ (number of nodes) \tcp*[r]{This function finds an edge and neighborhoods}
search an edge $e_{ij} \in E$ such that removal of $e_{ij}$ creates two subtrees $T_1$ and $T_2$ of $T$ with almost $\frac{1}{2}d$ nodes each\;
find $N(i)$ and $N(j)$\;
\Return [$e_{ij}$, $N(i)$, $N(j)$]
}
\textbf{End} FindEdge
\end{algorithm}

Following definitions are required to prove that Algorithmic Bound is correct.
\begin{definition}[Correlation decay property] \label{def2}
The Correlation Decay Property (CDP) states that the absolute value of the correlation coefficient between any two nodes decreases as the distance (the number of edges along the path between two nodes) between them increases \cite{F.Tan}.
\end{definition}
The dominant crossover event in tree-structured GGMs is defined in \cite{F.Tan}, \cite{Tavass}. The effect of this crossover event is as follows.
\begin{definition}[Impact of dominant errors]\label{def3}
An edge $e_{ij}$ is replaced with one of the candidate false edges: node $i$ is connected to one of the neighbors of node $j$ or vice versa.
\end{definition}

\subsubsection{Analysis of Algorithmic Bound}
First the time complexity of Algorithmic Bound (Algorithm \ref{algorithm2} and Algorithm \ref{algorithm3}) is discussed, and then proof of Algorithmic Bound correctness is provided by showing the validity of upper bound which is tighter than Theorem \ref{theorem2}.

\noindent \textbf{Time Complexity:} The overall time complexity of Algorithmic Bound (Algorithm 2 and Algorithm 3) is $\mathcal{O}(d)$ where $d$ is the number of nodes in a tree, which is dominated by the Break Function.

\noindent Time Complexity of Function Break: This function recursively breaks the tree with $d$ nodes in lines 10-11 of Algorithm \ref{algorithm3} where at each iteration the tree becomes almost half, hence, it takes $\mathcal{O}(\log d)$ time. While line 5 of Algorithm \ref{algorithm3} takes $\mathcal{O}(d)$ time due to FindEdge function. It has $\mathcal{O}(d)$ time complexity overall.

\begin{thm}[Algorithmic Bound on incorrect recovery probability] \label{theorem3}
Algorithmic Bound (Algorithm \ref{algorithm2}  and Algorithm \ref{algorithm3}) gives the valid upper bound on the incorrect tree structure recovery probability $Pr(\hat{T}_p \neq T_p)$, and it has $\mathcal{O}(d)$ time complexity where $d$ is the number of nodes in a tree graph.
\end{thm}
\begin{proof}
  Please see Appendix \ref{append5} for the proof of this theorem.
\end{proof}
